Formal Analysis of V2X Revocation Protocols

Research on vehicular networking (V2X) security has produced a range of security mechanisms and protocols tailored for this domain, addressing both security and privacy. Typically, the security analysis of these proposals has largely been informal. However, formal analysis can be used to expose flaws and ultimately provide a higher level of assurance in the protocols. This paper focusses on the formal analysis of a particular element of security mechanisms for V2X found in many proposals: the revocation of malicious or misbehaving vehicles from the V2X system by invalidating their credentials. This revocation needs to be performed in an unlinkable way for vehicle privacy even in the context of vehicles regularly changing their pseudonyms. The REWIRE scheme by Forster et al. and its subschemes BASIC and RTOKEN aim to solve this challenge by means of cryptographic solutions and trusted hardware. Formal analysis using the TAMARIN prover identifies two flaws with some of the functional correctness and authentication properties in these schemes. We then propose Obscure Token (OTOKEN), an extension of REWIRE to enable revocation in a privacy preserving manner. Our approach addresses the functional and authentication properties by introducing an additional key-pair, which offers a stronger and verifiable guarantee of successful revocation of vehicles without resolving the long-term identity. Moreover OTOKEN is the first V2X revocation protocol to be co-designed with a formal model.

==> figures/fig_PRESERVE_vSec.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.95\textwidth]{PRESERVE_vSec}
\caption{Abstract PRESERVE vehicle OBU security architecture~\cite{PRESERVE:D13}}
\label{fig:img:vSec}
\end{figure}

==> figures/fig_revocationAlgorithm.tex <==

\begin{algorithm}[H]
\floatname{algorithm}{\otoken Revocation Protocol}
% \renewcommand{\thealgorithm}{}
\begin{algorithmic}[1]
\STATE $V_j$ : Change from $SK_{Ps_i(V_j)}$ , $PK_{Ps_i(V_j)}$ to $SK_{Ps_i+1(V_j)}$ , $PK_{Ps_i+1(V_j)}$.
\STATE $RA\rightarrow{V_j}$ : Receive \osrreq message broadcast from $RA$.
\STATE $V_j$ : Decrypt \osrreq with $PK_{RA}$ to acquire $\sigma_{Ps_i(V_j)}$.
\STATE $V_j$ : Attempt to decrypt $\sigma_{Ps_i(V_j)}$ with $LTK_{V_j}$; to get $SK_{O_{Ps_i(V_j)}}$\\{\bf OR Failure}.
\STATE $V_j$ : Delete all $SK_{Ps_i(V_j)}$ , $PK_{Ps_i(V_j)}$.
\STATE $V_j\rightarrow{RA}$ : Create, encrypt and send \osrconf to $RA$.
\STATE $RA$ : Verify \osrconf with $PK_{O_{Ps_i(V_j)}}$.
\end{algorithmic}
\caption{Steps to revoke Vehicle $V_j$}
\label{fig:alg:revoke}
\end{algorithm}

==> sec_tands/tamarin.tex <==
\subsection{\tamarin}
\label{sec:rp:tamarin}
%
We model and analyse all three protocols, the \basic and \rtoken protocols
and our new \otoken protocol in~\Sref{sec:otoken} using the \tamarin prover.
The \tamarin prover is a symbolic analysis tool that is based on multiset rewriting
and first order logic. It supports logical connectives (\texttt{|, \&,
==>, not,} \dots) and quantifiers (\texttt{All, Ex}).
A multiset rewriting system defines a transition system and rules define how the
system can transition to a new state. The rules have sequences of facts as left-hand
sides, action labels, and right-hand-sides. Facts are of the form $F(t_1,\ldots, t_k)$
for a fact symbol $F$ and terms $t_i$. The left-hand-sides determine the state
required to execute the rule, the action labels represent transitions occurring,
and the right-hand-sides determine the resulting state. Messages are broadcast on
the network and consumed via an \texttt{Out} fact on the right-hand-side and
\texttt{In} fact on the left-hand-side. Protocol rules also use fixed unary fact
symbols $Fr$ to obtain fresh names on the left-hand-side. Protocols in \tamarin are
written in terms of rules and axioms. Axioms are specified properties in \tamarin
models that restrict the sequences of transitions.
% \todo[author=Frank]{The previous discussion of Tamarin could be clearer.}
%
%It supports logical connectives (\texttt{|, \&,
%==>, not,} \dots) and quantifiers (\texttt{All, Ex}). Protocols in \tamarin are
%written in terms of rules and axioms.  Rules define how transitions can be applied
%to evolve to a new state in the context of the behaviour of the protocol. Rules
%in \tamarin consists of three parts: premise, action labels and conclusion. The
%premise defines the state required to execute the rule which are expressed in
% terms of facts, the action labels represent
%transitions occurring, and the conclusion determines the resulting state.
%Messages are broadcast on the network and consumed via \texttt{Out} and
%\texttt{In} facts.
%The protocols investigated in this paper will be modelled by such transition
%rules, and also by the events
%%\texttt{Commit} and \texttt{Running} which are included to support the
%%authentication analysis as defined by Lowe~\cite{Lowe}.
%Axioms are specified properties in \tamarin models
%that restrict the sequences of transitions.
%\todo[author=Frank]{The previous discussion of Tamarin could be clearer.}

\tamarin has numerous built-in security theories that abstractly support common
cryptographic functions. For example, in this paper we use the {\it signing}
built-in which models a signature scheme. It provides the function symbols
\texttt{sign} and \texttt{verify} such that digital signatures can be verified
using the equation \texttt{verify( sign( m, sk ), m, pk( sk ) ) = true}.

Desired properties of the protocols are expressed as proof goals using first order logic
where quantification identifies specific timepoints over which the properties
hold. For example, \texttt{e @ \#i} expresses that the event \texttt{e} in a transition
occurs at timepoint \texttt{i} denoted by the \texttt{\#}-prefix.

Analysis of protocols is over an unbounded number of instances that makes it
suitable for an arbitrary number of vehicles. The analysis is performed in the
context of an attacker trying to manipulate communication. \tamarin provides
built-in support for a Dolev-Yao~\cite{DBLP:journals/tit/DolevY83} style network
attacker, i.e., an attacker who can eavesdrop on messages, broadcast on the
network, make new deductions and send messages but cannot decrypt messages unless
(s)he has the correct key.
